Gap Opening and Inner Disk Structure in the Strongly Accreting Transition Disk of DM Tau

Large inner dust gaps in transition disks are frequently posited as evidence of giant planets sculpting gas and dust in the disk, or the opening of a gap by photoevaporative winds. Although the former hypothesis is strongly supported by the observations of planets and deep depletions in gas within the gap some disks, many T Tauri stars hosting transition disks accrete at rates typical for an undepleted disk, raising the question of how gap opening occurs in these objects. We thus present an analysis of the structure of the transition disk around the T Tauri star DM Tau, which is strongly accreting ($\sim 10^{-8.3}~\mathrm{M}_\odot~ \mathrm{yr}^{-1}$) and turbulent ($\alpha=0.078 \pm 0.02$). Using the DALI thermochemical code, we fit disk models to simultaneously reproduce the accretion rate, high level of turbulence, the gas traced by ALMA band 6 observations of $^{12}$CO, $^{13}$CO, and C$^{18}$O J=2--1 lines, and the observed dust emission from the mm continuum and spectral energy distribution. We find a shallow depletion in gas surface density of $\sim 10$ relative to the outer disk and a gas rich inner disk is consistent with the observations. The planet mass of $<1$ M$_\mathrm{Jup}$ implied by the gap depth is in tension with predictions for dust trapping in a highly viscous disk, which requires a more massive planet of of $\sim10$M$_\mathrm{Jup}$. Photoevaporative models including a dead zone can qualitatively reproduce some features of the DM Tau disk, but still struggle to explain the high accretion rates and the observed mm continuum flux.

==> table_disk_geo.tex <==
\begin{deluxetable*}{cchhcc}
\tablecaption{Disk geometry}
\label{tab:disk_geo}
% \tablehead{\colhead{Name} & \colhead{Distance\tablenotemark{a}} & \colhead{Spectral Type} & \colhead{$T_\text{eff}$} & \colhead{Luminosity} & \colhead{Mass} & \colhead{A$_\textrm{V}$} & \colhead{$\dot{M}$} \\ \colhead{ } & \colhead{(pc)} & \colhead{ } & \colhead{(K)} & \colhead{($L_\sun$)} & \colhead{$M_\odot$} & \colhead{ } & \colhead{($\log_{10}(M_\sun/\text{yr}))$}}
\tablehead{\colhead{Distance (pc)} & \colhead{Disk Center (ICRS J2000)} & \nocolhead{$R_\text{inner}$ (au)} & \nocolhead{$R_\text{cav}$ (au)} & \colhead{i} ($^{\circ}$)  & \colhead{PA} ($^{\circ}$)} 
\startdata
145 & 04:33:48.749 +18.10.09.640 & 7.5 \pm 0.3 & 21 & $35.2 \pm 0.7$ & $157.8 \pm 1.0$ \\
\enddata
\tablecomments{References: Distance \citep{GaiaCollaboration2018}; DM Tau Geometry CITE KUDO; J1852 geometry - see section \ref{app:cont_fits} of the appendix. {\color{red} ERROR BARS FOR J1852 SEEM VERY SMALL, CHECK FITTING PROCEDURE. DISK STRUCTURE IS VERY CLEAN THOUGH SO MAYBE THEY ARE OKAY?}
}
\end{deluxetable*}

==> table_stellar_properties.tex <==
\begin{deluxetable*}{cccccccchh}
\tablecaption{Stellar Properties}
\label{tab:stellar}
% \tablehead{\colhead{Name} & \colhead{Distance\tablenotemark{a}} & \colhead{Spectral Type} & \colhead{$T_\text{eff}$} & \colhead{Luminosity} & \colhead{Mass} & \colhead{A$_\textrm{V}$} & \colhead{$\dot{M}$} \\ \colhead{ } & \colhead{(pc)} & \colhead{ } & \colhead{(K)} & \colhead{($L_\sun$)} & \colhead{$M_\odot$} & \colhead{ } & \colhead{($\log_{10}(M_\sun/\text{yr}))$}}
\tablehead{\colhead{Distance (pc)} & \colhead{Spectral Type} & \colhead{$T_\text{eff} (K)$} & \colhead{Luminosity ($L_\sun$)} & \colhead{Mass ($M_\odot$)} & \colhead{A$_\textrm{V}$} & \colhead{$\dot{M}$ ($\log_{10}(M_\sun/\text{yr}))$} & \nocolhead{i ($^{\circ}$)}   & \nocolhead{PA ($^{\circ}$)} } 
\startdata
145 & M1 & 3580 & 0.24 & 0.39 & 0.5 & -8.30 & 10 & 10 \\
\enddata
\tablecomments{References: Distance \citep{GaiaCollaboration2018}; stellar mass, luminosity, spectral Type, Teff \citep{Francis2020}; Accretion rate \citep{Manara2014}.
\tablenotetext{a}{}
}
\end{deluxetable*}
